Robust Pre-Training by Adversarial Contrastive Learning

Recent work has shown that, when integrated with adversarial training, self-supervised pre-training can lead to state-of-the-art robustness In this work, we improve robustness-aware self-supervised pre-training by learning representations that are consistent under both data augmentations and adversarial perturbations. Our approach leverages a recent contrastive learning framework, which learns representations by maximizing feature consistency under differently augmented views. This fits particularly well with the goal of adversarial robustness, as one cause of adversarial fragility is the lack of feature invariance, i.e., small input perturbations can result in undesirable large changes in features or even predicted labels. We explore various options to formulate the contrastive task, and demonstrate that by injecting adversarial perturbations, contrastive pre-training can lead to models that are both label-efficient and robust. We empirically evaluate the proposed Adversarial Contrastive Learning (ACL) and show it can consistently outperform existing methods. For example on the CIFAR-10 dataset, ACL outperforms the previous state-of-the-art unsupervised robust pre-training approach by 2.99% on robust accuracy and 2.14% on standard accuracy. We further demonstrate that ACL pre-training can improve semi-supervised adversarial training, even when only a few labeled examples are available. Our codes and pre-trained models have been released at: https://github.com/VITA-Group/Adversarial-Contrastive-Learning.

==> sections/1-intro.tex <==
\section{Motivation, Background and Related Works}


This paper is to demonstrate the value of contrastive-style unsupervised pre-training, for adversarially robust deep learning. Our methodology is deeply rooted in the recent surge of ideas from self-supervised learning (esp. as pre-training \cite{chen2020adversarial}), contrastive learning (esp. \cite{chen2020simple}), and adversarial training (esp. the unlabeled approaches \cite{stanforth2019labels}). We review those relevant fields to gradually unfold our rationale.

% pre-training
% -> traditional role: improve accuracy and stablize training
% -> recently (tianlong): carefully designed proxy tasks 
% -> lately, contrasting is good
% -> feature consistency is recently founded not naturally meet (consistency training, natural fragile)
% -> we conjecture contrasting is a good proxy and explore and find it good too


% Supervised training of deep neural networks requires massive, labeled datasets, which may be unavailable and costly to assemble \cite{hinton2006fast,bengio2007greedy,raina2007self,vincent2010stacked}. Self-supervised and unsupervised training techniques attempt to address this challenge by eliminating the need for manually labeled data. Representations pretrained through self-supervised techniques enable fast fine-tuning to multiple downstream tasks, and lead to better generalization and calibration  \cite{liu2019towards,mohseni2020self}. Examples of tasks proven to attain high accuracy through self-supervised pretraining include position predicting tasks (\textit{Selfie} \cite{trinh2019selfie}, \textit{Jigsaw} \cite{noroozi2016unsupervised, carlucci2019domain}), rotation predicting tasks (\textit{Rotation} \cite{gidaris2018unsupervised}), and a variety of other perception tasks \cite{criminisi2004region,zhang2016colorful,dosovitskiy2015discriminative}.


% The labeling and sample efficiency challenges of deep learning are further exacerbated by vulnerability to adversarial attacks. For example, Convolutional Neural Networks (CNNs), are widely leveraged for perception tasks, due to high predictive accuracy.  However, even a well-trained CNN suffers from high misclassification rates when imperceivable perturbations are applied the input~\cite{Kurakin2016AdversarialML, moosavi2016deepfool}. As suggested by \cite{schmidt2018adversarially},  the sample complexity of learning an adversarially robust model with current methods is significantly higher than that of standard learning. Adversarial training (AT) \cite{madry2017towards}, the state-of-the-art model defense approach, is also known to be computationally more expensive than standard training (ST). 



% Why SS, review SS methods in adversarial learning
% Convolutional Neural Networks (CNNs) have achieved tremendous success in many visual tasks. Systems based on it are deployed to various applications. Some of them are safety-critical, like medical diagnostics \cite{shen2017deep} and antonymous driving \cite{bojarski2016end}. However, it is shown that CNNs are suffering from serious vulnerability \cite{goodfellow2014explaining}. Imperceivable perturbations
% are even able to skew the prediction of a well-trained network to be an arbitrary value. 

% Adversarial Training, the state-of-the-art method to defense the vulnerability \cite{madry2017towards}, requires much more sample complexity to generalize than Standard Training \cite{zhai2019adversarially}. One approach to address this challenge is to employ Self-Supervised Training. Previous work \cite{chen2020adversarial} investigates different pretext Self-Supervised methods (i.e. Selfie \cite{trinh2019selfie}, Jigsaw \cite{noroozi2016unsupervised, carlucci2019domain}). While Selfie achieves significant improvement on both accuracy and robustness, Jigsaw would hurt accuracy while improving robustness, showing the important role of the type of employed Self-Supervised method. 

%However, the types of self-supervised method that has been explored are very limit. They are all pretext tasks designed based on heuristics. Recently, another branch of self-supervised methods based on contrastive learning showing promising performance on ST.
% Despite this, in AT context, the types of SS methods that been explored are very limited. Particularly, the contrastive learning based SS methods are still not investigated, though it has shown promising results, achieving the state-of-the-art performance in ST.

% Recently, the family of Self-Supervised methods based on Contrastive Learning is becoming popular, achieving statue-of-the-art in many benchmarks \cite{chen2020simple}, which leads to a natural question: \textit{Can Contrastive Learning further stimulate the potential power of Self-Supervised Training in Adversarial Training?}
%However, the contrastive learning based SS methods are still not investigated in AT context.

% In this work, we extensively investigate multiple strategies for incorporating Contrastive Learning as pre-training. We demonstrate the great potential of contrastive learning in Adversarial Training. (e.g. in CIFAR-10, the best strategy improves both standard accuracy and robust accuracy by [XX.XX\%, XX.XX\%] compared to state-of-the-art adversarial pre-training method.)

% Moreover, given Contrastive Learning's promising results on leveraging the unlabeled data, we also extend it to Unsupervised Adversarial Training \cite{stanforth2019labels}. It shows a \textbf{large improvement} on utilizing the unlabeled data. Specifically, one CIFAR-10, it leads to XX\% on standard accuracy and XX\% on robust accuracy with 200K unlabeled data compared to the previous state-of-the-art method.

%To this end, the Self-supervised training techniques are employed and proven to be significantly helpful for AT. \cite{tianlong} compared three self-supervised techniques (Selfie, Jigsaw and Rotation). Big performance gap is found among them. This further motivates the designing for more sophisticated self-supervised technique.

% Why contrastive learning: 1. SOTA method in unsupervised method. 2. some reasons of being good.
% Contrastive learning, the state-of-the-art self-supervised method in ST, . However, it still remains unclear about whether it is helpful for AT. In this work, we propose a simple adversarial contrastive learning framework (simAdvCLR), which further improve previous self-supervised training in many aspects.  

% The questions to explore for contrastive learning
% To summarize, our contributions are:
% \begin{itemize}
% \item We demonstrate for the first time that Contrastive Learning can be incorporated as a competitive Self-Supervised method in Adversarial Training and consistently contribute to robustness on multiple datasets.
%self-supervised robust pretrained models leveraged for adversarial fine-tuning on 10\% labeled data can yield comparable robustness to a model adversarially trained with 100\% labeled data. Compared to previous semi-supervised state-of-the-art in adversarial training, pretrained model can improve \textbf{7.55\%} robust accuracy and \textbf{2.63\%} standard accuracy.
% \item We show that Contrastive Learning can better utilize unlabeled data for improving robustness.
% \item When employing the same network architecture, on the CIFAR-10 dataset, our method surpasses the state-of-the-art methods for Adversarial Training, Unsupervised Adversarial Training, and Self-Supervised Training.
% \end{itemize}

\subsection{Classical Pre-Training and Self-Supervision}

 Training a supervised deep network from scratch requires tons of labeled data, whose annotation costs can be prohibitively high. Utilizing unlabeled data e.g., by various unsupervised or semi-supervised learning techniques, is thus of booming interests. One promising option is to first pre-train a feature representation using unlabeled data, which is later fine-tuned for down-stream tasks using (few-shot) labeled data. In general, pre-training is discovered to stabilize the training of very deep networks \cite{hinton2006fast,bengio2007greedy}, and usually improves the generalization performance, especially when the labeled data volume is not high. Such \textit{pre-training \& fine-tuning} scheme further facilitates general task transferability and few-shot learnability of each down-steam task. Therefore, pre-trained models have gained popularity in computer vision \cite{kornblith2019better}, natural language processing \cite{devlin2018bert} and so on.


Unsupervised pre-training initially adopted the reconstruction loss or its variants \cite{bengio2007greedy,vincent2010stacked}. Such simple, generic loss learns to preserves input data information, but not to enforce more structural  priors on the data. Recently, self-supervised learning emerges to train unsupervised dataset in a supervised manner, by framing a supervised learning task in a special form to predict only a subset of input information using the rest. The self-supervised task, also known as \textit{pretext} task, guides us to a supervised loss function, leading to learned representations conveying structural or semantic priors that can be beneficial to downstream tasks. Classical pretext tasks include position predicting \cite{trinh2019selfie}, order prediction \cite{noroozi2016unsupervised, carlucci2019domain}, rotation prediction \cite{gidaris2018unsupervised}, and a variety of other perception tasks \cite{dosovitskiy2015discriminative,zhang2016colorful}.

\subsection{Self-Supervised Pre-Training Helps Adversarially Robust Learning}

The labeling scarcity is further amplified when we come to adversarially robust deep learning ~\cite{moosavi2016deepfool}, i.e., to training deep models that are not fooled by maliciously crafted, although imperceivable perturbations. As suggested in \cite{schmidt2018adversarially},  the sample complexity of adversarially robust generalization is significantly higher than that of standard learning. Recent results \cite{stanforth2019labels,alayrac2019labels,carmon2019unlabeled} advocated unlabeled data to be a powerful backup for training adversarially robust models as well, by using unlabeled data to form an auxiliary loss (e.g., a label-independent robust regularizer or a pseudo-label loss).

Only lately, researchers start linking self-supervised learning to adversarial robustness. \cite{hendrycks2019using} proposed a multi-task learning framework that incorporates a self-supervised objective to be co-optimized with the conventional classification loss. The latest work \cite{chen2020adversarial}  introduced adversarial training \cite{madry2017towards} into self-supervision, to provide general-purpose robust pretrained models for the first time. The authors found these robust pretrained models can benefit the subsequent fine-tuning in two ways: i) boosting final model robustness; and ii) saving the computation cost if continuing with adversarial fine-tuning. Comparing the two, \cite{chen2020adversarial} adopts the \textit{pre-training \& fine-tuning} scheme and is more plug-and-play and easy-to-use with different down-stream tasks: we hence choose to follow this setting.


\begin{figure*}\centering
  \includegraphics[width=0.5\columnwidth]{images/intro.pdf}
  \caption{Illustration of the performance of out approach. Black circle is the baseline method: end-to-end adversarial training. Blue circle is the previous state-of-the-art pre-training method. Red circle is the best proposed method in terms of robustness.}
  \label{fig:teaser}
\end{figure*}



\subsection{Contrastive Learning Brings Feature Consistency that Fits Adversarial Robustness}


Handcrafted pretext tasks \cite{noroozi2016unsupervised, carlucci2019domain,trinh2019selfie,gidaris2018unsupervised} rely on heuristics to design, and thus could limit the generality of the learned representations. An emerging new category of self-supervised methods, called \textit{contrastive learning}, has shown recently shown great promise. The main idea underlying contrastive learning is to learn unsupervised representation by minimizing the distance between positive pairs; meanwhile many methods would also maximize the distance between negative pairs. 

Contrastive Predictive Coding (CPC) \cite{oord2018representation} first advocated to translate a generative modeling problem to a classification problem. Their contrastive loss enforces the model to classify the future representation among a set of unrelated “negative” samples. Built on CPC, \cite{wu2018unsupervised,he2019momentum} introduced memory banks to store past negative examples for dictionary look-up. More model architecture variants were presented in \cite{misra2019self,bachman2019learning,henaff2019data}. Very recently, a simple yet elegant framework called \textit{SimCLR} was presented in \cite{chen2020simple}. for contrastive learning of visual representations, by maximizing agreement between differently augmented views of the same sample via a contrastive loss in the latent space. As the state-of-the-art contrastive learning (and unsupervised pre-training) framework, SimCLR can even surpass the fully-supervised AlexNet \cite{krizhevsky2012imagenet} when fine-tuned on only 1\% of the labels.

Essentially, SimCLR empowers the unsupervised feature with  \textit{invariance} to specified data transformations. Such feature-level invariance is well-known to be desirable for standard generalization of CNNs, yet is often not met by state-of-the-art CNNs \cite{zhang2019making,kayhan2020translation}. Therefore, enforcing \textit{consistency} w.r.t data augmentations has been shown effective for unsupervised learning \cite{hu2017learning,ye2019unsupervised,xie2019unsupervised}. 

Although all contrastive learning literature \cite{oord2018representation,wu2018unsupervised,he2019momentum,chen2020simple} merely discussed their boost on the standard generalization, we realize that  the feature consistency (as a result of contrasting) is intuitively valuable for robustness too. One cause of adversarial fragility could be attributed to the non-smooth feature space near samples, i.e., small input perturbations can result in large feature variations and even label change. Enforcing consistency during training, w.r.t. to either random or adversarial perturbations, has been thus shown to immediately help adversarial robustness \cite{stanforth2019labels,zhai2019adversarially,carmon2019unlabeled}. A closely relevant work \cite{hendrycks2019augmix} showed that a combination of stochasticity and diverse augmentations, plus a feature divergence consistency loss, improved the robustness and uncertainty estimates of fully-supervised image classifiers. 

The above observations constitute our conjecture that contrastive learning could be a superior option for adversarial pre-training to other classical self-supervision tasks. Compared to those adopted by \cite{chen2020adversarial}, the feature consistency appears to be more directly targeted to the robustness issue. 





% Handcrafted pretext tasks contains solving jigsaw puzzles \cite{noroozi2016unsupervised, carlucci2019domain}, relative patch prediction \cite{trinh2019selfie} and rotation prediction \cite{gidaris2018unsupervised}. Contrastive Learning based methods learn representation by minimizing the distance between positive pairs while maximizing between negative pairs \cite{chen2020simple}. 
% Recent works investigate contrastive learning from many dimensions: the positive and negative pairs setting \cite{hjelm2018learning}, model architectures \cite{misra2019self,bachman2019learning,henaff2019data} and the loss function \cite{oord2018representation}. Benefits from these findings. SimCLR \cite{chen2020simple}, the state-of-the-art framework, can even surpass the previous label-supervised  state-of-the-art: Alexnet \cite{krizhevsky2012imagenet}. 


\subsection{Our Contributions: Adversarial Contrasting} 

%As self-supervised tasks are demonstrated to help the prediction accuracies of deep supervised classifiers, it remains yet to be explored how they might affect their adversarial robustness.  An approach is offered in \cite{hendrycks2019using}, by %treating  incorporating the self-supervised task as a complementary objective, which is co-optimized with the conventional classification loss through the method of AT \cite{madry2017towards}. Their co-optimization approach presents scalability challenges, and does not enjoy the benefits of pretrained embeddings.  Further, it leaves many unanswered questions, especially with respect to efficient tuning, which we tackle in this paper.




%To address this,  Self-Supervised Training techniques are proposed. When serving as a pre-training, it boosts the down-stream tasks by improving prediction generality with fewer data \cite{liu2019towards}. Recently, Self-Supervised Training even surpasses previous state-of-the-art method: AlexNet \cite{krizhevsky2012imagenet} with 100x less labels on ImageNet \cite{chen2020simple}.

%The label insufficient problem is becoming more serious when it comes to the vulnerability of adversarial attacks. For instance, imperceivable perturbations are even able to skew the prediction of a well-trained network to be an arbitrary value \cite{moosavi2016deepfool,kurakin2016adversarial}. While methods like Adversarial Training (AT) \cite{madry2017towards} greatly relieve the vulnerability, they desire higher label complexity than Standard Training (ST) for satisfactory generalizability \cite{schmidt2018adversarially}. Thus, Self-Supervised Training is leveraged in Adversarial Training. With carefully designed pretext tasks, \cite{xie2019adversarial} and \cite{chen2020adversarial} shows improvement in both generalizability and convergence speed. A popular explanation for the improvement is these pretext tasks can enforce the modeling of image structural information such as shape \cite{xie2019adversarial}.

%However, the structural information is not enough given the local feature can also improve the robustness \cite{song2019robust}. Therefore, for learning more comprehensive features, we propose to employ the Contrastive Learning based Self-Supervised method, which enforces the invariance between different augmented images. Benefiting from the flexibility of Contrastive Learning, different features can be learned with different augmentations employed. For example, the structural and local information can be learned by enforcing consistency between different colorized images and image crops from different locations, respectively. Moreover, by encouraging the agreement with adversarial perturbed images, robustness can also be gained more directly.

%While consistency idea is also discussed in \cite{kannan2018adversarial,carmon2019unlabeled,zhai2019adversarially}, they don't employ large augmentations, leaving the structural and local information not enforced. \cite{hendrycks2019augmix} considers the consistency between augmented images, but the effect of adversarial robustness is not discussed. Here, we focus on learning more comprehensive features through enforcing consistency.

Given the state-of-the-art adversarial robustness and accuracy achieved by the pre-training scheme \cite{chen2020adversarial}, our goal is to further push the boundary: \textit{how much more robustness we could gain by improving pre-training}? Our solution is based on several innovative modifications of SimCLR \cite{chen2020simple}, inspired by its direct impact on enforcing the desirable feature consistency. The resultant unsupervised pre-training framework, called \textit{Adversarial Contrasting}, is thoroughly discussed in Section \ref{sec:method}. 

On CIFAR-10/CIFAR-100, we extensively benchmark our pre-trained models on two adversarial fine-tuning settings: \textit{fully-supervised} (using all training data and their labels) and \textit{semi-supervised} (using all training data, but only partial/few shot labels). Our pre-training leads to establishing the new state-of-the-art bars in terms of both robust and standard accuracies. For example, in the fully-supervised case, adversarial contrasting yields XX.XX\% robustness and XX.XX\% standard accuracy improvements over the previous best... For semi-supervised setting, our approach bypasses the previous state-of-the-art method \cite{stanforth2019labels} by a margin of XX.XX\% robustness and XX.XX\% standard accuracy, with only XX\% labeled data on the CIFAR-10.




% In this work, we propose the Adversarial Contrasting, the framework of Contrastive Learning based Self-Supervised methods for Adversarial Training.  we start with conjecturing multiple Adversarial Contrasting methods. When fine-tuning. Our best strategy improves the previous state-of-the-art method by XX.XX\% and XX.XX\% on both accuracy and robustness with 0.XX\% training time. Moreover, we further extend it to Unsupervised Adversarial Training. It surpasses the previous state-of-the-art method \cite{stanforth2019labels} with only XX\% labeled data on the CIFAR-10.

% To summarize, our contributions are:
% \begin{itemize}
% \item We propose the Adversarial Contrasting, the first Contrastive Learning based Self-Supervised framework for Adversarial Training.
% \item We show that Adversarial Contrasting can better utilize unlabeled data for improving robustness.
% \item When employing the same network architecture, on the CIFAR-10 dataset, our method surpasses the state-of-the-art methods for Adversarial Training, Unsupervised Adversarial Training, and Self-Supervised Training.
% \end{itemize}


\Ziyu{shorten this part to: short intro, related works, discussion}
